RA-PbRL: Provably Efficient Risk-Aware Preference-Based Reinforcement Learning

Reinforcement Learning from Human Feedback (RLHF) has recently surged in popularity, particularly for aligning large language models and other AI systems with human intentions. At its core, RLHF can be viewed as a specialized instance of Preference-based Reinforcement Learning (PbRL), where the preferences specifically originate from human judgments rather than arbitrary evaluators. Despite this connection, most existing approaches in both RLHF and PbRL primarily focus on optimizing a mean reward objective, neglecting scenarios that necessitate risk-awareness, such as AI safety, healthcare, and autonomous driving. These scenarios often operate under a one-episode-reward setting, which makes conventional risk-sensitive objectives inapplicable. To address this, we explore and prove the applicability of two risk-aware objectives to PbRL : nested and static quantile risk objectives. We also introduce Risk-AwarePbRL (RA-PbRL), an algorithm designed to optimize both nested and static objectives. Additionally, we provide a theoretical analysis of the regret upper bounds, demonstrating that they are sublinear with respect to the number of episodes, and present empirical results to support our findings. Our code is available in https://github.com/aguilarjose11/PbRLNeurips.

==> kwise.tex <==
\section{ICVaR Preference-based RL with n-wise Comparisons}

In the previous section, we proposed a provably efficient algorithm that achieves near-optimal regret for PbRL. However, this framework may not be apt for certain PbRL scenarios where sampling trajectories can be reserved and people can compare multiple trajectories and the agent receives the feedback of each pairs. Take clinical trials as an example: different medical treatments can be assessed concurrently, with feedback manifesting as pairwise comparisons or rankings among them. The imperative for risk-awareness in such scenarios is undeniable, too. Simultaneously, the capacity to store trajectories enables multiple comparisons to be made between the same pair of trajectories by human evaluators. Therefore, it is essential to develop a rational comparison strategy to enhance efficiency in this context. To address this, we introduce a novel setting in this section, named ICVaR-PbRL$^+$, which allows for n-wise comparisons. This setting extends the original ICVaR-PbRL, encompassing broader applications. We detail the setup and learning objectives of ICVaR-PbRL$^+$, followed by an outline of the algorithm and its theoretical underpinnings.

\subsection{Algorithm}
The algorithm, formally delineated in Algorithm \ref{al2}, parallels the framework of Algorithm \ref{al1} in its structure. The key distinctions lie in two points. Firstly, the construction of confidence sets and exploration bonus is different. Secondly, the algorithm involves a judgment process to determine whether $m$ times comparison should be made between two trajectories. 

\begin{algorithm}[h]

  \caption{ICVaR-PBRL$^+$}
  \begin{algorithmic}[1]
  \label{al2}
    \INPUT episode $K$, step $H$, the number of trajectories for each episode $n$.
    %\STATE Initialize the estimated state transition model and utility model: $\widehat{P}_0$, $\widehat{r}_0$, the transition and utility confidence range coefficient : $\beta_{P,0}$, $\beta_{r,0}$. 
    \STATE Execute arbitrary policies $\pi_{0, 1}, \pi_{0, 2},\ldots,\pi_{0,n}$ for one episode, respectively, and then observe the preference $o_{1, i, j}$ between $\tau_{1, i}$ and $\tau_{1, j}$ for all $(i, j) \in\{(i, j) \mid 1 \leq i<j \leq n\}$.
    \FOR{$k=1 \cdots K$}
    
    %\STATE $\bar{r}_{k} \leftarrow \arg \max _{r \in r_B} \mathcal{L}_{k-1}$
    \STATE Calculate the reward estimation $\widehat{r}_{k}$ using Eq.\ref{reward estimate1}. 
    \STATE Update the confidence set $\mathcal{B}^r_{k}$ using Eq.\ref{reward confidence1}.
    \STATE Update the transition distance function $D_k(\cdot,\cdot)$ using Eq. \ref{prob11} and Eq.\ref{prob3}.
    \STATE Calculate the possibility estimation $\widehat{\mathbf{P}}_{k}$ using Eq.\ref{estimate prob1}.
    \STATE Calculate the reward $ b^{r}_{k,h}$ and transition bonus $ b^{\mathbf{P}}_{k,h}$ using Eq. \ref{reward bonus} and Eq. \ref{transition bonus}.
    \STATE Update transition confidence set $\mathcal{B}^{\mathbf{P}}_{ k}$ using Eq. \ref{possibility confidence1}.
    
     %\STATE $\Bar{\mathcal{P}_{k}} \sim N(\bar{\mathbb{P}}_{k}, \sigma_{\mathrm{p}}^2 \Sigma_{k-1}^{-1})$
    %\STATE $\widehat{\mathcal{P}}_{k+1, h}=\left\{\mathbb{P}^{\prime} \in \mathcal{P}: \sum_{i=1}^k \operatorname{Dist}_{i, h}\left(\mathbb{P}^{\prime}, \widehat{\mathbb{P}}_{i, h}\right) \leqslant \widehat{\gamma}^2\right\} $ \\//Construct the confidence set
    
    \STATE Update policy set $S_t$ using Eq. \ref{policyset}
     \STATE Compute $\pi_{k, 1}, \pi_{k, 2},\ldots,\pi_{k,n}$ using Eq. \ref{choosepolicy1}
      \STATE Execute arbitrary policies $\pi_{k, 1}, \pi_{k, 2},\ldots,\pi_{k,n}$ for one episode, respectively, and then observe $\tau_{k, i}$ and $\tau_{k, j}$ for all $(i, j) \in\{(i, j) \mid 1 \leq i<j \leq n\}$
      \FOR{$i=1\cdots n$}
        \FOR{$j=i+1 \cdots n$}
        
            \IF{$|\hat{r}_k(\tau_i)-\hat{r}_k(\tau_j)|$\\$\leq |b^{r}_{k,h}(\tau_i-\tau_j)|+b^{p}_{k,h}(\tau_i)+b^{p}_{k,h}(\tau_j)$}
            \STATE$ \mathbb{I}_{k,i,j}=1$
            \STATE Query comparison oracle $m$ times on $\tau_i$ and $\tau_j$, received feedback $o_{i,j} \in [m]$.
            \ELSE 
            \STATE $ \mathbb{I}_{k,i,j}=0$
            \ENDIF
      \ENDFOR
      \ENDFOR
    \ENDFOR
  \end{algorithmic}
\end{algorithm}


In alignment with the PbRL setting, we employ least-squares regression to estimate the reward function as follows:
\begin{align}
\label{reward estimate1}
\widehat{r}_k(\cdot)=\arg\min \sum\limits_{t=1}^{k-1}\sum\limits_{i=1}^n \sum\limits_{j=i+1}^n \mathbb{I}_{k,i,j}\left({\sigma}(r(\tau_{t, i}) -r(\tau_{t, j}))-o_{t}\right)^2 
\end{align}

And then we construct the reward confidence set:
\begin{align}
\label{reward confidence1}
\mathcal{B}^{r}_{ k}= 
 \begin{cases}
\mathcal{R}, \; K=0\\
\left\{ r^\prime(\cdot) \middle| \sum\limits_{t=1}^{k-1}\sum\limits_{i=1}^n \sum\limits_{j=i+1}^n\mathbb{I}_{k,i,j}[(\hat{\sigma}_k- \sigma^\prime)
(\tau_{t, i},\tau_{t, j})\right]^2 \leq \beta_{r,k} (\delta)]\}, K\geq1
\end{cases}
\end{align}

where $(\hat{\sigma}_k-\sigma^\prime)(\tau_{1},\tau_{ 2})=\sigma(\widehat{r}_k(\tau_{1})-\widehat{r}_k(\tau_{2}))-\sigma(r^\prime(\tau_{1})-r^\prime(\tau_{2}))$. %\yujie{$\beta$!!!!}

And we estimate the transition kernel as follows:
\begin{align}
\label{estimate prob1}   \hat{\mathbf{P}}_k=\arg\min_{\mathbf{P}\in\mathcal{P}} D_{k}(\mathbf{P}^{\prime}, \delta_{k-1}).
\end{align}
Where $ D_{k}(\cdot)$ is a distance function defined as follows:
\begin{align}\label{prob11}
D_k(\mathbf{P}_1,\mathbf{P}_2)=\sum_{i=1}^2\sum_{t=1}^{k-1}\sum_{h=1}^H| \langle \mathbf{P}_1-\mathbf{P}_2, \mathbf{V}_{h}(s_{i},a)|^2
\end{align}
Then we constructed transition confidence set as follows:
\begin{equation}
\label{possibility confidence1}
\begin{small}
    \mathcal{B}^{\mathbf{P}}_{ k}=
    \begin{cases}
     \mathcal{P}, K=0\\
      \left\{\mathbf{P}^{\prime} \mid D_{k}\left(\mathbf{P}^{\prime}, \hat{\mathbf{P}}_k\right) \leq \beta_{\mathbf{P},k}(\delta)\right\} , K \leq1 .
    \end{cases}
    \end{small}
\end{equation}


Also we use reward bonus in Eq.\ref{reward bonus} and transition bonus Eq.\ref{transition bonus} to encourage exploration. Meanwhile, we employ the  near-optimal policy set described in Eq. \ref{policy set}.

Finally, we choose the exploratory polices $\left(\pi_{k, 1}, \pi_{k, 2}, \cdots, \pi_{k, n}\right)$ that can maximize the pairwise uncertainty as follows:
\begin{align}
\label{choosepolicy1}
& \left(\pi_{k, 1}, \pi_{k, 2}, \cdots, \pi_{k, n}\right)=\underset{\pi_1, \pi_2, \cdots, \pi_n \in s_k}{\arg \max } \sum_{i=1}^n \sum_{j=i+1}^n \nonumber\\
&\mathbb{E}_{\tau_1 \sim\left(\hat{\mathcal{P}_k}, \pi_{i}\right), \tau_2\sim\left(\hat{\mathcal{P}_k}, \pi_j\right)}\left(b^{\mathbf{P}}_{k}(\tau_1)+b^{\mathbf{P}}_{k}(\tau_2)\right)\nonumber\\
   &+\mathbb{E}_{\tau_1 \sim\left(\hat{r_k}, \pi_i\right), \tau_2 \sim\left(\hat{r_k}, \pi_j\right)}\left(b^{r}_{k}(\tau_1,\tau_2)\right) .
\end{align}

\begin{theorem}\textbf{(Regret Minimization (RM))}
\label{k-wise regret}
For some positive constant $\delta \in (0,1]$, the regret of Algorithm \ref{al1} is bounded when the number of episodes $K$ satisfies the inequalities $H \sqrt{d_\mathbf{P} nK \log \left(\frac{H N\left(\mathcal{F}_{P}, \frac{1}{nK}, \|\cdot\|_{\infty}\right)}{\delta}\right)} \geq \alpha^H$ and $\frac{1}{\lambda m\alpha^H}\sqrt{d_r K \log \left(H N\left(\mathcal{F}_{\mathcal{R}}, \frac{1}{n^2K},\|\cdot\|_{\infty}\right) / \delta\right)}\geq KH$.
\begin{align}
  \operatorname{Regret}(K)
    \leq O\left(\frac{1}{1-\alpha}\left(\frac{\alpha^{-H-1}-\alpha}{1-\alpha}-H\alpha\right)\Delta^\prime_{\mathbf{P}}+O\left(\frac{1}{\lambda\alpha^H}\Delta^\prime_{r}\right)\right)
\end{align}    
Otherwise, 
\begin{align}
    \operatorname{Regret}(K)\leq KH .
\end{align}
Where $\Delta^\prime_{\mathbf{P}}=\sqrt{d_{\mathbf{P}} nK \log \left(H N\left(\mathcal{F}_{P}, 1 / (Kn),\|\cdot\|_{\infty}\right) / \delta\right)}$ and $\Delta^\prime_r=\frac{1}{m}\sqrt{d_r K \log \left(H N\left(\mathcal{F}_{\mathcal{R}}, 1 / (Kn^2),\|\cdot\|_{\infty}\right) / \delta\right)}$.  Here $d_\mathbf{P}=\operatorname{dim}_E(\mathcal{P}, 1 / K)$ and $d_r=\operatorname{dim}_E(\mathcal{R}, 1 / K)$ are the eluder dimension in Definition \ref{eluder}.

\end{theorem}
From the error introduced by $\Delta_r$, it is evident that in scenarios where the reward function exhibits increased complexity, appropriately augmenting the number of comparisons \(m\) for each pair can enhance efficiency more effectively within a total number of comparisons on the order of \(\sim O(mK)\).



% \huazheng{Choice of $\alpha$? Regret order? Explain the result. See ICVaR-RL paper as an example -- they always have a paragraph after each major theorem to explain it. Also any novelty in proof we want to mention for this theorem or previous lemmas?}

%\begin{theorem}
%    \textbf{Best Policy Identification (BPI)}
%\end{theorem}


 


